If At First You Don't Succeed: Extended Monitorability through Multiple Executions

This paper studies the extent to which branching-time properties can be adequately verified using runtime monitors. We depart from the classical setup where monitoring is limited to a single system execution and investigate the enhanced observational capabilities when monitoring a system over multiple runs. To ensure generality in our results, we focus on branching-time properties expressed in the modal mu-calculus, a well-studied foundational logic that is used by state-of-the-art model checkers. Our results show that the proposed setup can systematically extend previously established monitorability limits for branching-time properties. We then validate our results by instantiating them to verify actor-based systems. We also prove bounds that capture the correspondence between the syntactic structure of a property and the number of required system runs.

==> preamble/drawing.tex <==
% Configure libraries to be imported by TikZ.
\usetikzlibrary {
  calc,
  shadows,
  shapes,
  arrows,
  arrows.meta,
  chains,
  matrix,
  decorations.pathmorphing,
  decorations.pathreplacing,
  decorations.text,
  patterns,
  fit
}

% Define custom TikZ arrow tips for processes.
\tikzset{
  triangle/.tip={Triangle[open, scale=0.9]},
  drone/.tip={Stealth[scale=0.68]},
  vector/.tip={Latex[scale=0.68]},
  into/.tip={To[scale=0.77]},
  parenthesis/.tip={Parenthesis[reversed, scale=0.86]},
  bars/.tip={Bar[sep=1pt]Bar},
}

% Define custom TikZ line styles for processes.
\tikzset{
  fork/.style={draw, -triangle, dotted},
  tell/.style={-vector},
  2 way tell/.style={vector-vector},
  expo/.style={draw, parenthesis-into, wave},
  exit/.style={draw, -bars, dotted}
}

\pgfdeclaremetadecoration{middlezigzag}{straight}{
    \state{straight}[switch if less than=\pgfmetadecorationsegmentlength to final,
                  width=\pgfmetadecoratedpathlength/2 - \pgfmetadecorationsegmentlength/2 ,
                  next state=zigzag] {
        \decoration{curveto}
    }
    \state{zigzag}[width=\pgfmetadecorationsegmentlength,
                   next state=final] {
        \decoration{zigzag}
    }
    \state{final}{
        \decoration{curveto}
        \beforedecoration{\pgfpathmoveto{\pgfpointmetadecoratedpathfirst}}
    }
}

\pgfdeclaremetadecoration{presnake}{pre}{
    % \state{straight}[switch if less than=\pgfmetadecorationsegmentlength to final,
    %               % width=\pgfmetadecoratedpathlength/2 - \pgfmetadecorationsegmentlength/2 ,
    %               width=\pgfkeysvalueof{/pgf/decoration/pre length},
    %               next state=snake] {
    %               \decoration{moveto}
    % }
    % \state{snake}[width=\pgfmetadecoratedpathlength/2 - \pgfmetadecorationsegmentlength/2,

    \state{pre}[width=0, next state=snake]{
      \beforedecoration{\pgfpathmoveto{\pgfpointmetadecoratedpathfirst}}
    }
    \state{snake}[width=\pgfmetadecorationsegmentlength/3,
                   next state=final] {
                   \decoration{snake}
        % \afterdecoration{\pgfpathmoveto{\pgfpointmetadecoratedpathlast}}
    }
    \state{final}{
        \decoration{curveto}
        \beforedecoration{\pgfpathmoveto{\pgfpointmetadecoratedpathfirst}}
    }
}

% Middle zigzag idea from here.
% https://tex.stackexchange.com/questions/33162/tikz-decoration-with-1cm-zigzag-in-the-middle-of-a-link/33182
% https://tex.stackexchange.com/questions/18617/tikz-draw-only-a-certain-central-length-of-a-given-path/18623

% Define custom TikZ decorations and styles.
\tikzset{
  pre snake/.style={
    decoration={
      presnake,
      segment length=3, 
      amplitude=0.4, 
      post length=0.3em, 
      pre length=0.3em
    },
    decorate
  },
  wave/.style={
    decoration={
      snake, 
      segment length=3, 
      amplitude=0.4, 
      post length=0.3em, 
      pre length=0.3em
    },
    decorate
  },
  fray/.style={
    decoration={
      zigzag, 
      segment length=3, 
      amplitude=0.8      
    },
    decorate
  },
  small fray/.style={
    decoration={
      zigzag, 
      segment length=3, 
      amplitude=0.04em
	  },
	  decorate
  },
  tear/.style={
    decoration={
      zigzag, 
      segment length=6, 
      amplitude=1.8,
	  }, 
	  decorate
  },
  elevate/.style={
    drop shadow,
	  fill=white
  }
}

% Define custom TikZ shapes.
\tikzset{
  label/.style={
    font=\scriptsize\itshape,
    inner sep=0.4em
  },
  circ/.style={
    circle, 
    draw,
    minimum width=4em,
    minimum height=4em,
    font=\footnotesize,
    inner sep=0.1em,
    align=center
  },
  process/.style={
    rectangle,
    draw,
    minimum width=2em,
    minimum height=4em,
    font=\footnotesize,
    align=center,
    text depth=-0.08em,
    inner sep=0.3em
  },
  decision/.style={
    diamond, 
    draw,
    minimum width=5em,
    minimum height=5em,
    font=\footnotesize,
    align=center, 
    node distance=2.5cm, 
    inner sep=0.1em
  },
  cloud/.style={
    draw, 
    ellipse,
    node distance=3cm, 
    minimum height=2em,
    font=\footnotesize, 
    align=center, 
    inner sep=0.3em
  },
  monitor/.style={
    process,
    rounded corners=0.2em
  },
  small monitor/.style={
    process,
    circle,
    rounded corners=0.2em
  },
  tape/.style={
    font=\tiny\ttfamily,
    minimum size=1.2em,
    draw,
    text centered,
    %   text height=1.5ex,
    text height=0.2em, 
    text width=0.9em,
    inner sep=0,
    outer sep=0,
    % text depth=-0.3em,
  },
	nstep/.style={
		align=center,
		minimum width=0.7em,
		minimum height=0.6em,
		inner sep=0.1em,
		outer sep=0em,
		font=\sffamily\scriptsize,
		draw,
		semithick,
		% text=white,
		fill=white,
    rounded corners=0.3em,
    % text depth=-0.1em
	},
% 	cnumb/.style={
% 		circle,
% 		align=center,
% 		minimum size=0.8em,
% 		inner sep=0.05em,
% 		outer sep=0em,
% 		font=\sffamily\tiny,
% 		draw,
% 		% text=white,
% 		fill=white
% 	},
% 	strikef/.style={
%     semithick,
%     draw=tblgray,
%     strike out,
%     inner sep=0pt,
%     minimum width=1em,
%     minimum height=1em
% 	},
% 	strikeb/.style={
%     semithick,
%     draw=tblgray,
%     strike out,
%     inner sep=0pt,
%     minimum width=1em,
%     minimum height=1em,
% 		rotate=90
% 	},
% 	crossn/.style={
%     semithick,
%     draw=tblgray,
%     cross out,
%     inner sep=0pt,
%     minimum width=1em,
%     minimum height=1em
% 	},
  heavyarrow/.style={
    single arrow,
    draw,
    fill=black,
    minimum width=1em,
    minimum height=4em,
    inner sep=0ex,
    single arrow head extend=0.2em,
  },
  cross/.style={
    cross out,
    draw,
    semithick, 
    % minimum size=2*(#1-\pgflinewidth), 
    inner sep=0pt, 
    outer sep=0pt,
    minimum width=0.4em,
    minimum height=0.4em
  }
}

% Define global lengths for use in TikZ figures.
\newlength{\gap}
\setlength{\gap}{0.4em}

==> preamble/graphic.tex <==
%!TEX root=../main.tex

%:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::
% Additional TikZ configuration.
%:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::

% Imported TikZ libraries.
\usetikzlibrary {
  matrix,
  shapes,
  arrows,
  shadows,
  calc,
  chains,
  decorations.pathmorphing,
  decorations.text,
  arrows.meta,
  patterns,
  fit
}


%:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::
% Graphic objects.
%:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::

% Custom shapes.
\tikzset{
  label/.style={
    font=\scriptsize\itshape,
    inner sep=0.4em
  },
  point/.style={
    circle,
    fill=black,
    text width=0.3em,
    inner sep=0
  },
  state/.style={
    circle,
    text width=0.8em,
    inner sep=0.1em,
    text depth=0.08em,
    draw,
    font=\scriptsize
  }
}
